A Video is Worth 256 Bases: Spatial-Temporal Expectation-Maximization Inversion for Zero-Shot Video Editing

This paper presents a video inversion approach for zero-shot video editing, which models the input video with low-rank representation during the inversion process. The existing video editing methods usually apply the typical 2D DDIM inversion or naive spatial-temporal DDIM inversion before editing, which leverages time-varying representation for each frame to derive noisy latent. Unlike most existing approaches, we propose a Spatial-Temporal Expectation-Maximization (STEM) inversion, which formulates the dense video feature under an expectation-maximization manner and iteratively estimates a more compact basis set to represent the whole video. Each frame applies the fixed and global representation for inversion, which is more friendly for temporal consistency during reconstruction and editing. Extensive qualitative and quantitative experiments demonstrate that our STEM inversion can achieve consistent improvement on two state-of-the-art video editing methods. Project page: https://stem-inv.github.io/page/.

==> fig_tex/all-frame.tex <==
\begin{figure}[t]
  \centering  \includegraphics[width=1.0\linewidth]{figs/all-frame5.pdf}
  \vspace{-0.7cm}
\caption{Reconstruction results with different inversion.}
\vspace{-0.4cm}
  \label{fig:all-frame}
\end{figure}




==> fig_tex/psnr.tex <==
\begin{figure*}[t]
  \centering  \includegraphics[width=0.9\linewidth]{figs/psnr.pdf}
  \vspace{-0.3cm}
  \caption{Quantitative evaluation of the 8-frame reconstructed video with PSNR and SSIM, where TokenFlow and STEM-TokenFlow use the typical DDIM reconstruction, while FateZero and STEM-FateZero additionally leverage attention fusion during reconstruction~\cite{fatezero}.}
  \label{fig:psnr}
\end{figure*}

==> related.tex <==
\section{Related Work}
\noindent{\textbf{Text-dirven image generation and editing.}}
Image generation is a fundamental task in computer vision. 
There have been many studies on image generation based on GANs~\cite{gan,stylegan}, VAE~\cite{vae,vqvae}, auto-regressive Transformers~\cite{VQVAE2,esser2021taming,gafni2022make,wu2022nuwa,yu2022scaling}, and flow~\cite{kingma2018glow}. Recently, diffusion models~\cite{ddpm,ddim} have merged as a popular choice for text-to-image (T2I) generation since their stunning results.
DALLE-2~\cite{dalle} and Imagen~\cite{imagen} can generate realistic images by conditioning in text embeddings from large language models~\cite{clip,raffel2020exploring}, where cascaded diffusion models are used to scale up image resolution gradually.
Stable Diffusion~\cite{ldm} applies diffusion models in the latent space of powerful pre-trained auto-encoders in VQ-GAN~\cite{esser2021taming}, achieving training and inference on limited resources.


For text-driven image editing, ControlNet~\cite{controlnet} enhances large pre-trained text-to-image diffusion models with
task-specific image conditions, such as depth map, canny edge~\cite{canny}, and human pose. Besides, a number of studies explore text-based interfaces for content manipulation~\cite{sine,instructpix2pix}, style transfer~\cite{kwon2022diffusion,zhang2023inversion}, and generator domain adaption~\cite{kim2022diffusionclip}. 
% Moreover, a group of methods~\cite{custom-diffusion,dreamartist,fastcomposer,dreambooth,textual-inversion,celeb} conduct personalized text-guided image editing and synthesize novel renditions of one or several given subjects in different contexts by tuning models with given samples.




 


 

\noindent{\textbf{Text-dirven video generation and editing.}}
Text-to-video (T2V) turns to generate corresponding videos based on the given prompt. Imagen-Video~\cite{imagen_video} proposes a cascaded video diffusion model that sequentially increases the resolution of generated videos via a series of super-resolution diffusion models. Make-A-Video~\cite{make-a-video} proposes to fine-tune the T2I model for video generation, where a spatiotemporally factorized diffusion model is designed.




In terms of text-driven video editing, Tune-A-Video~\cite{tune} proposes to conduct one-shot video tuning for videos, while inflating 2D-UNet and replacing self-attention as sparse causal attention for temporal modeling.
Fatezero~\cite{fatezero} and Pix2Video~\cite{pix2video} apply attention maps to model temporal consistency, which can be regarded as an implicit manipulation way. 
Besides, Rerender-A-Video~\cite{rerender} and Video-ControlNet~\cite{videocontrolnet} use optical flow for frame-wise constraints.
Further, several methods~\cite{edit_a_video,video-p2p,vid2vid-zero} have been aware that the inaccurate DDIM inversion would lead to accumulated errors during the denoising process, and thus turn to Null-text inversion~\cite{null}. However, this optimization-based inversion takes 2 minutes per frame using an A100 GPU, which is unfavourable in real applications.




In contrast to previous methods, we propose to overhaul DDIM inversion into STEM inversion, where we reformulate the input video representation as a low-rank basis set by the EM algorithm, which harvests a fixed spatial-temporal context from the entire video for each frame, rather than exploring time-varying one like existing DDIM does. Besides, the row-rank representation reduces the complexity in self-attention layers. 





 % and we hope that STCN can be adopted as the new and efficient backbone for future works.


% The spatial-temporal correspondence is established in editing process. specifically, for each to be edited frame $X_i$ ($i \in{1,2,...n}$), Pix2video leverages both $i-1$ (previous) and $i=1$ (the first) frames as reference to perform self-attention feature injection.
% TokenFlow~\cite{tokenflow} exploits the semantic similarity of duffusion features across frames, and conduct linear interpolation to modify those inaccurate features (tokens). 



%Null text Inversion
% Edit-A-Video~\cite{edit_a_video}
% Video-P2P~\cite{video-p2p}
% Vid2vid-zero~\cite{vid2vid-zero}



%Studies on image generation have appeared several times in literature.
%Diffusion models are generative models characterized by a forward and reverse Markov process.

==> table_tex/rebuttal_length.tex <==
\begin{table}
\footnotesize
\centering 
\begin{tabular}{l|c|c|c|c|c}
\toprule  
Length
&{8}
&{16}
&{32} 
&{64}
&{128}\\
\hline
PSNR &32.702  &\textbf{33.279}  &33.197   &33.058    &32.751  \\
\hline
SSIM  &0.9836 &\textbf{0.9854}  &\textbf{0.9854}    &0.9851   &0.9843 \\
\bottomrule
\end{tabular}
\vspace{-2mm}
\caption{Results of STEM Inv with various video lengths.}
\label{tab:length}
\vspace{-2mm}
\end{table}


==> table_tex/rebuttal_resolution.tex <==
\begin{wraptable}{l}{4.2cm}
\captionsetup{font=footnotesize}
\footnotesize
\vspace{-0.08cm}
\setlength{\tabcolsep}{0.8mm}{} 
\begin{tabular}{l|c|c|c|c}
\toprule  
Size 
&{$384^2$}
&{$512^2$}
&{$768^2$} 
&{$1024^2$}\\
\hline
PSNR &29.558 &33.767   & 34.813    &\textbf{35.668}  \\
\hline
SSIM  &0.9743 &0.9847  &0.9901 &\textbf{0.9902}  \\
\bottomrule
\end{tabular}
\vspace{-0.32cm}
\captionsetup{font=small}
\caption{Results of STEM Inv with various video resolutions.}
\label{tab:resolution}
\vspace{-0.45cm}
\end{wraptable}
